On Reverse Elastic Channels and the Asymmetry of Commitment Capacity under Channel Elasticity

Commitment is an important cryptographic primitive. It is well known that noisy channels are a promising resource to realize commitment in an information-theoretically secure manner. However, oftentimes, channel behaviour may be poorly characterized thereby limiting the commitment throughput and/or degrading the security guarantees; particularly problematic is when a dishonest party, unbeknown to the honest one, can maliciously alter the channel characteristics. Reverse elastic channels (RECs) are an interesting class of such unreliable channels, where only a dishonest committer, say, Alice can maliciously alter the channel. RECs have attracted recent interest in the study of several cryptographic primitives. Our principal contribution is the REC commitment capacity characterization; this proves a recent related conjecture. A key result is our tight converse which analyses a specific cheating strategy by Alice. RECs are closely related to the classic unfair noisy channels (UNCs); elastic channels (ECs), where only a dishonest receiver Bob can alter the channel, are similarly related. In stark contrast to UNCs, both RECs and ECs always exhibit positive commitment throughput for all non-trivial parameters. Interestingly, our results show that channels with exclusive one-sided elasticity for dishonest parties, exhibit a fundamental asymmetry where a committer with one-sided elasticity has a more debilitating effect on the commitment throughput than a receiver.

==> converse.tex <==
\section{Converse}

==> response.tex <==


\parskip 3mm
\parindent 0mm

\newcommand{\X}{{\mathbf X}}
\newcommand{\aec}[1]{\noindent {\it Guest Editor's comment: #1}}
\newcommand{\rfc}[1]{\noindent {\it \underline{Reviewer's comment:} #1}}
\newcommand{\rc}[1]{\noindent {\it \underline{Reviewer's comment:} #1}}
\newcommand{\res}[1]{\noindent {\underline{Authors' Response:} #1}}
\newcommand{\todo}[1]{\textcolor{blue}{To Do: #1}}
\newcommand{\think}{\textcolor{red}{To think}}

\newpage

\setcounter{page}{1}
%\addtocounter{page}{-20}
{\Large\bf Authors' response to the reviewers' comments for submission JSAC-PIR-2021 (\#68: 1570731937) \\ ``On Reverse Elastic Channels and the Asymmetry of Commitment Capacity under Channel Elasticity''}

We thank the guest editor and the reviewers for their comments and suggestions.
We have made changes to incorporate their suggestions.
Below we provide a point-by-point response and indicate 
the changes made. For convenience, we reproduce the comments of the
reviewers in {\it italics}, while our response is in normal font.
All page numbers refer to the revised draft. 

\vspace{5mm}
{\Large\bf Response to the Guest Editor's comments}

\vspace{5mm}
\aec{Both reviewers recommend acceptance of this manuscript, subject to minor revisions. The authors are asked to carefully incorporate the points raised by the reviewers.}

\res{  
We thank the guest editor and the reviewers for their encouraging comments and generally positive evaluation of our work. We  sincerely appreciate the extremely detailed, extensive and insightful comments by reviewers and we have tried our best to incorporate appropriate changes.    }


\vspace{5mm}
{\Large\bf Response to the comments of Reviewer 1}
%rev1

\vspace{5mm}
\rfc{
This paper characterizes the commitment capacity of reverse elastic channels, proving a recent conjecture (Claude Crépeau, Rafael Dowsley, Anderson C. A. Nascimento. On the Commitment Capacity of Unfair Noisy Channels. IEEE Transactions on Information Theory 66(6): 3745-3752, 2020).

The protocol for achieving the desired rate follows the approach of previous works, but the converse proof uses new ideas.

The results are all correct and the work obtained the commitment capacity of reverse elastic channels, solving an open question regarding the use of those channels for cryptographic purposes. 

No weaknesses.
}

\res{We thank the reviewer for summarizing the key contributions of this work succinctly here. We find the reviewer's positive feedback on our work extremely satisfying.} 


\vspace{5mm}
{\Large\bf Response to the comments of Reviewer 2}
%rev2

\vspace{5mm}
\rc{The paper tightly characterizes the commitment capacity of reverse elastic channels. \\
-- A reverse elastic channel (REC) is a binary symmetric channel with noise characteristic delta. An adversarial sender can reduce the noise characteristic to gamma. \\
-- The commitment functionality allows the sender to commit to a bit-string without revealing it to the receiver. The receiver is guaranteed that the sender is bound to one particular bit-string. 
-- The capacity of an REC is the ratio of the committed bit-string to the number of REC invocations. 

Tight capacity results are exciting and suitable for the venue, and they are of broader interest. The techniques are interesting and I have verified most of the technical details in the paper and am reasonably confident of their correctness.
\begin{enumerate}[(+)]
\item The upper bound to the commitment capacity is innovative. It is surprising that the commitment capacity of REC is strictly smaller than the commitment capacity of elastic channels (EC). It was an exciting open problem left open by the recent work of Crepeau-Dowsley-Nascimento, 2020. \\
\item The capacity-achieving hashing-based commitment protocol is also (sufficiently) elegant.
\end{enumerate}
}

\res{
We thank the reviwer for the detailed summary of our work. We particularly appreciate the reviewer's studious examination of our manuscript (as can be seen from the extensive feedback by the reviewer which we respond to  in detail later). It is our strong belief that the  many  comments/suggestions, both technical as well as  in writing style, offered by the reviewer (accompanied by insightful remarks) have greatly enhanced the quality of our presentation now. In particular, these have helped us bring more focus on the  novelty of our contributions and refine the writing in several parts of this manuscript.
It is particularly pleasing to us that the reviewer finds our results suitable to this journal and of broad interest to this community. }



\rc{
(No significant weaknesses) There are minor presentation issues and some additional presentation-related suggestions that are elaborated in detail later. 
}

\res{We are happy to note that the reviewer has not found any significant weaknesses in our work. We are extremely thankful to the reviewer for pointing out presentation issues with the manuscript, where some parts may require additional discussion and/or clarification. We have tried to address these in the revision and we hope that the changes are satisfactory. 

In the following, we provide a short point-by-point bulletized response; here reviewer comments \emph{in italics} are immediately followed by short authors' responses in normal font. In some cases, detailed responses to certain reviewer comments are again provided later for clarification and completeness. 

}


%\begin{enumerate}[(*A)]

\noindent$(*A)$ \emph{The definition of rate needs additional clarifications. For example, a definition that also considers implementing reliable channels from RECs was not incorporated. More about it in the full review.} \\
\noindent$\bullet$  We agree with the reviewer that alternate notions are meaningful. Thanks for pointing this out. We have now included a footnote to bring this point out more clearly (see footnote~\ref{foot:rate} on pg.~\pageref{page:rate}), and emphasize our specific definition of rate in this work. We discuss this point later in the review again.\\
\noindent$(*B)$ \emph{Why figure 1 only considers one $s$ and not an adversary who adaptively sets the noise characteristic?  Damgard-Kilian-Salvail proved that any adversary using $s > \gamma$ can be simulated by 
another adversary using $s = \gamma.$ So, why is that substitution not made (without loss of generality)?} \\
%
\noindent$\bullet$  The reviewer is correct that for the REC$[\gamma,\delta]$ one can consider a more generalized setting where unlike an adversary with a \emph{static} choice of $s_i=s, \ \forall i\in[n]$ where $s\in[\gamma,\delta],$ one can assume an \emph{adaptive} adversary which can induce  a possibly \emph{time-varying} channel transition probability with potentially different values $s_i\in[\gamma,\delta],$ $\forall i\in[n].$ When writing the manuscript we too deliberated on such a presentation of the model. However, we decided to go ahead with a static (instead of the adaptive) adversary in Fig.~1 to establish a direct parallel with the classic REC$[\gamma,\delta]$ as defined in Khurana-Maji-Sahai, EUROCRYPT'16, where the model allowed a fixed $s\in[\gamma,\delta]$ for all instances in $[n]$. Our proof brings out the fact that such an adaptive action does not benefit a malicious party which will always default a choice of $s=\gamma$; this was also showed by Damgard-Kilian-Salvail-EUROCRYPT'99 as the reviewer mentions. We now discuss this important implication (that the commitment capacity remains the same) for adaptive malicious parties   immediately after the main theorem in more detail; we thank the reviewer for pointing this out.\\ 
\noindent$(*C)$ \emph{The keys $K_A$ and $K_B$ in figure 1: Are they arbitrarily distributed or chosen according to some distribution?}\\
\noindent$\bullet$  Alice and Bob have access to private randomness and the keys $K_A$ and $K_B$ capture the random actions and/or transmissions that Alice and Bob can effect privately. We  have now presented this in detail in the manuscript (see the problem setup on pg.~\pageref{page:protocol}). We hope this brings clarity to the presentation which might have been previously missing.
%\end{enumerate}




\rc{
Summary.\\
The paper makes a tight characterization of the commitment capacity of reverse elastic channels. The result is exciting and suitable for the venue, and it should be of broader interest. I have verified most of the technical details in the paper and am reasonably confident of their correctness. 

Noise that is beyond the control of parties is an incredible facilitator of cryptography. For example, random samples from noisy channels facilitate secure multi-party computation (MPC), an incredibly sophisticated cryptographic primitive that allows parties to compute securely over their private data. A central functionality in MPC is the commitment functionality, which forces malicious parties to behave honestly during the protocol execution. This work studies the rate of the commitment functionality using partially compromised noisy channels, vis-a-vis the ratio of the number of bits being committed to the number of noisy-channel invocations. 

Suppose the noise characteristic of a noisy channel, for example, a binary symmetric channel, can be adversarially controlled by the parties. The space of parameters for these partially compromised noisy channels enabling MPC has been the object of extensive research. Damgard-Kilian-Salvail (EUROCRYPT 1999) introduced unfair noisy channels (UNC) where both the sender and the receiver can control the noise characteristic of the channel, and an adversarial party can make it more reliable. Khurana-Maji-Sahai (EUROCRYPT 2016) introduced elastic channels (EC) where only an adversarial receiver can make the channel more reliable.  This work studies the commitment rate/capacity for reverse elastic channels (REC) where an adversarial sender can make the channel more reliable. 

An REC$[\gamma,\delta]$ is a BSC with noise characteristic delta. An adversarial sender can reduce the noise characteristic in the range $[\gamma, \delta]$ arbitrarily. 

This paper makes two contributions. 
\begin{enumerate}[(1)]
\item Proves a converse result proving an upper bound on the rate of the commitment functionality for REC. 
\item Presents a construction matching the upper bound. 
\end{enumerate}

Formally, the paper studies a system where parties have access to
\begin{enumerate}[(1)]
\item reliable communication channels
\item REC channel. 
\end{enumerate}
}

\res{We once again thank the reviewer for the extremely positive assessment of our contribution in this work. We thank the reviewer for summarizing our problem of commitment over an REC  as well as bring in  the necessary context (via UNCs) for why unreliable channels (RECs are one of them) have been of interest to the community in recent times (essentially since the key work of Damgard-Kilian-Salvail-EUROCRYPT'99 on UNCs). }

\rc{
A commitment functionality is an interactive functionality with two phases, the commitment phase, and the reveal phase. All bit-strings should be equally likely to be the committed string at the end of the commitment phases (hiding property). However, the sender cannot open to a different string during the opening phase (binding property).\\
Remark: This definition is a game-theoretic definition of security that this paper considers (in contrast to a simulation-based definition). For simulators with unbounded computational power, this game-theoretic definition coincides with the simulation-based security definition.  In this line of work, it is typical to consider the game-based definition instead of the simulation-based security definition because they admit clean mathematical models. 
}

\res{We thank the reviewer for pointing this out, and agree that mentioning this would help a potential reader. We have now explicitly mentioned this fact in the introduction on page~\pageref{def:UNC} under the footnote~\ref{foot:game}, and included some appropriate references. }

\rc{
Remark: The paper should justify why the rate/capacity of the commitment functionality is defined using the definition "ratio of committed string to the number of invocations of REC." For example, another alternative model is to consider realizing the reliable communication channel using REC and then taking the ratio of the committed string with the number of REC invocations. The definition used in this work has also been used in prior works and is adequate. However, a clarification that alternative definitions of rate are possible shall be informative. (More intuition provided in the perspective paragraph below).}

\res{As we mentioned in response to an earlier comment, we agree with the reviewer about different notions of rate. We thank the reviewer for pointing this out. We have now added a discussion on pg.~\pageref{page:protocol} to bring this out more clearly.} 

\rc{
Remark: In figure 1, the model states that the adversarial sender fixes the noise characteristic to $s$. The model can, for example, consider the case where the adversary sets each REC invocation adaptively. However, we know that the view of an adversary using the noise parameter $s$ can be simulated by another adversary who uses the noise parameter gamma. Damgard-Kilian-Salvail provides this reduction. So, without loss of generality, one can consider the adversary who uses $s=\gamma$ in every REC invocation. The paper can start with this assumption. 
}

\res{We agree with the reviewer. This has been addressed in the revision as already discussed earlier. Please refer to our response to the bulletized set of  changes earlier.}

\rc{
Clarification: The paper should clearly state in Figure 1 whether the keys $K_A$ and $K_B$ are arbitrarity distributed or are randomly distributed? 
} 

\res{This has been addressed in the revision as already discussed earlier. Please refer to our response to the bulletized set of minor changes.}

\rc{
Perspective: The paper proves the surprising result that the commitment capacity of REC is smaller than the capacity of EC with identical parameters (proved by Crepeau-Dowsley-Nascimento, 2020). Observe that for honest but curious adversarial parties, REC and EC are equivalent because they are reversible (by using the one-time pad technique and increasing the communication over the reliable channel only). Thus, all efficiency measurements remain identical for REC and EC if they are agnostic to the communication complexity over the reliable channels. Therefore, the gap in the commitment capacity is fascinating against malicious parties. 
}

\res{We are extremely thankful to the reviewer for sharing this perspective. We find this comment particularly insightful as it helps present a different facet to our contribution; this was previously missing in our writing. We have now included a discussion immediately after the Remark~\ref{rem:pos} (see pg.~\pageref{page:curious}) where we discuss how the  \emph{honest-but-curious} model differs from the malicious model. In particularly, while the REC and EC offer identical commitment capabilities when parties are honest-but-curious; there is an asymmetric (w.r.t. Alice and Bob) degradation in the throughput when individual parties can maliciously control the channel.  }


\rc{Presentation Modularity. It will benefit the presentation of the construction protocol if the paper states its constructions in two steps. (1) commitment to a random bit-string, and (2) commitment to a particular bit-string. The construction of (2) from (1) uses the one-time pad technique, which the authors mention. One can refer to it as the "random self-reducibility" of the commitment functionality. The commitment to a random bit-string is much simpler and shall be more accessible to the readers. This reduction preserves the definition of commitment capacity used in this work. } 

\res{We thank the reviewer for suggesting the above two-step framework; the ``random-self-reducibility'' notion was not known to us earlier. In fact, the reviewer's comment reveals an interesting \emph{strengthening} of our soundness criterion. In the previous manuscript, our \emph{averaged-over-$C$}-soundness guarantee meant that soundness was guaranteed with high probability (i.e., for a `overwhelming fraction' of commit strings but not all). However, our achievability analysis  allows us to strengthen this criterion to a \emph{maximum-over-$C$}-soundness criterion, where we can guarantee soundness for any given commit string $C.$ We believe this is in the spirit of the reviewer's suggestion and thank the reviewer for pointing this out. We have now suitably modified our $\epsilon$-soundness criterion in~\eqref{eq:sound} in the revised manuscript. The rest of the analysis remains essentially the same as earlier. Also, the converse is still presented for the \emph{averaged-over-$C$}-soundness criterion; such a converse is \emph{stronger} as a rate upper bound under the weaker  (averaged) soundness criterion directly implies impossibility under the stronger (maximum) soundness criterion.
}



\rc{Minor comments in presentation.}

\res{We have addressed each of these in the revision. Thank you for a detailed reading to spot these. Our response (indicated as ``\emph{Auth.}'' follows the reviewer's suggestions (indicated as ``\underline{Rev.}'') in a sequential manner. 
\begin{description}
\item[\underline{Rev.}] \emph{"Often times" should be replaced either by "often" or by "oftentimes."} 
\item[\it{Auth.}] Thank you. We have made this change now.
\item[\underline{Rev.}] \emph{The definition of min-entropy in section II.A. is missing the "-log" term. }
\item[\it{Auth.}] We have corrected the error.
\item[\underline{Rev.}] \emph{Theorem 10: It will improve readability to clarify that the expression "(delta-gamma) / (1-2gamma)" is the noise characteristic such that when composed with BSC-gamma, one gets a BSC-delta channel. }
\item[\it{Auth.}] We have changed the presentation in Thm. 10 to clearly bring out the effective composition of BSC channels. We have also included a short discussion about  this in our remark.
\item[\underline{Rev.}] \emph{When bounding the rate R, ``$ZK_BM$'' should be ``$Z, K_B, M$'' in the first align* in the left column. }
\item[\it{Auth.}] Thank you for spotting this. We have made this change.
\item[\underline{Rev.}] \emph{The second align* below it should begin with ``$R \leq$'' instead of ``$R =$''.}
\item[\it{Auth.}] Yes, we have changed the equality to an inequality here.
\item[\underline{Rev.}] \emph{The description of the commit phase of the protocol should move the computation of "$\mathcal{L}(\by)$" (step C2) to the reveal phase. }
\item[\it{Auth.}] We have made this change now. We agree with this suggestion. 
\item[\underline{Rev.}] \emph{There is a global issue of ``[footnotemark][punctuation mark],'' which should be replaced by ``[punctuation mark][footnotemark]''.}
\item[\it{Auth.}] We thank the reviewer was pointing this out. We weren't aware of our `misuse' of the footnote referencing style; this will help us in our future writing endeavours too.
\end{description}
}




==> subsec_discussion.tex <==
We settle the conjecture for the commitment capacity of reverse elastic channel presented by Crepeau et.al in~\cite{crepeau2020commitment}.

For a given $\delta$ and $\gamma$, we can show that the commitment capacity of an elastic channel, $H(\gamma)$, is always greater than or equal to the commitment capacity of the reverse elastic channel $H(\delta) - H\left(\frac{\delta-\gamma}{1-2\gamma}\right)$. 
%It gives an interesting observation about the asymmetry of the commmitment protocols.
This illustrates that the asymmetry in adversarial powers of the committer and receiver, in that a malicious committer can wreak much more havoc than a malicious sender on the commitment rate.

The commitment capcity of the defined EC model is the same as that of the compound-BSC[$\gamma,\delta$], studied in~\cite{ncc21} where both Alice and Bob don't have any control over the channel. Further, the commitment capacity in the cases of EC and REC is higher than the commitment capacity over UNCs where either of the parties can act maliciously. This implies that restricting the malicious behaviour either of the parties results in high throughput and more the parties can act maliciously, more the rate goes down.\\ 
It's also quite interesting to note here that these noisy channels such as the UNC, EC, REC etc. may come under an umbrella of general unreliable channels where the restrictions at Alice's end or Bob's end could be more general in terms of mismatch and asymmetry in their controlling abilities over the noisy channel . It would be quite interesting to obtain the commitment capacity of such general unreliable channels. We seek to present this in our future work.
